GPRidge: Gaussian-process Accelerated Calculations of Minimum Energy Paths and First-order Saddle Points

GPRidge, a Gaussian-process (GP) library for accelerating calculations of minimum energy paths and first-order saddle points with compiled-language and Python bindings, is presented. An evaluation controller uses GP predictions to iteratively adjust the Cartesian coordinates of the atoms. The fitted GP energy surface and measured energies and forces pass from the path calculation to local refinement of the saddle point. New evaluations improve the surrogate and check the candidate geometry. For the molecular calculations, acceptance requires measured-force convergence and an independent Hessian with only one negative eigenvalue. A second negative eigenvalue triggers an escape and renewed refinement. The controller supports a joint inverse-distance GP for molecules and local GP residuals on periodic systems. Applications to the 24 Baker-Chan and 20 Birkholz-Schlegel molecular reactions using the Universal Model for Atoms (UMA-S-1.1), and to 72 Pt heptamer and island rearrangements on Pt(111) using a Morse potential, are presented. On matched Baker-Chan reactions, GPRidge uses 7.8- and 7.0-fold fewer energy-and-force evaluations than climbing-image nudged elastic band (CI-NEB) and off-path climbing-image nudged elastic band (OCI-NEB), respectively, reducing validation-inclusive CI-NEB time by 41%. All 20 Birkholz-Schlegel saddle points pass the independent index-one check, compared with 17 for the classical dimer method started from the same path maxima; on those 17 reactions, the GP dimer stage uses 6.4-fold fewer evaluations. All 72 Pt(111) paths meet the OptBench force criterion, with median evaluation counts of 30 and 23 for the heptamer and island problems, against 778 and 443 for CI-NEB.

==> figures/house_tikz.tex <==
\providecolor{RuhiTeal}{HTML}{004D40}
\providecolor{RuhiCoral}{HTML}{FF655D}
\providecolor{RuhiYellow}{HTML}{F1DB4B}
\providecolor{RuhiInk}{HTML}{1C2421}
\tikzset{
  gpr figure/.style={font=\footnotesize\sffamily, text=RuhiInk,
                     line cap=round, line join=round, >={Stealth[length=5pt]}},
  gpr note/.style={font=\scriptsize\sffamily, text=RuhiInk, align=center},
  gpr panel/.style={font=\footnotesize\sffamily\bfseries, text=RuhiInk,
                    anchor=north west, inner sep=0pt},
  gpr box/.style={draw=RuhiInk, line width=0.7pt, rounded corners=2pt,
                  fill=RuhiTeal!8, align=center, inner sep=4pt},
  gpr hot/.style={gpr box, fill=RuhiCoral!14, draw=RuhiCoral!80!black},
  gpr exit/.style={gpr box, fill=RuhiTeal!20},
  gpr entry/.style={gpr box, fill=RuhiYellow!22, draw=RuhiYellow!70!black},
  gpr arrow/.style={-{Stealth[length=5pt]}, line width=0.7pt, draw=RuhiInk},
  gpr axis/.style={->, line width=0.6pt, draw=RuhiInk!60},
}

